One-4-All: Neural Potential Fields for Embodied Navigation

A fundamental task in robotics is to navigate between two locations. In particular, real-world navigation can require long-horizon planning using high-dimensional RGB images, which poses a substantial challenge for end-to-end learning-based approaches. Current semi-parametric methods instead achieve long-horizon navigation by combining learned modules with a topological memory of the environment, often represented as a graph over previously collected images. However, using these graphs in practice requires tuning a number of pruning heuristics. These heuristics are necessary to avoid spurious edges, limit runtime memory usage and maintain reasonably fast graph queries in large environments. In this work, we present One-4-All (O4A), a method leveraging self-supervised and manifold learning to obtain a graph-free, end-to-end navigation pipeline in which the goal is specified as an image. Navigation is achieved by greedily minimizing a potential function defined continuously over image embeddings. Our system is trained offline on non-expert exploration sequences of RGB data and controls, and does not require any depth or pose measurements. We show that O4A can reach long-range goals in 8 simulated Gibson indoor environments and that resulting embeddings are topologically similar to ground truth maps, even if no pose is observed. We further demonstrate successful real-world navigation using a Jackal UGV platform.

==> background_backup.tex <==
\section{RELATED WORK}

The problem of robot navigation has been extensively studied in the literature \cite{thrun2005robotics}. In recent years there has been a growing trend towards image-based learning approaches also called \textit{experiental learning} \cite{Levine2023survey}. These approaches have the advantage of being able to reason about the navigability of both geometric and non-geometric concepts, such as tall grass in a field \cite{shah2021rapid}. In contrast, classic approaches that rely purely on the geometry of the environment through metric representations struggle with such concepts, leading to inefficient navigation plans \cite{wang2021survey}. 

Reinforcement Learning (RL) agents are a prominent example of experiential learning, which have been widely employed for image-based embodied navigation \cite{kuan2019memory, erik2019ddppo, rao2021endtoend}. While these approaches provide a sound solution to the navigation problem, RL policies are known to be data-hungry, with some \textit{offline} RL methods requiring up to 30 hours of training data \cite{shah2022revind}. Moreover, one of the key challenges of RL is their limited navigation capabilities over long horizons \cite{dulan2021challenges}.

To overcome the long horizon limitation, semi-parametric approaches utilize a topological memory \cite{Kuipers1988classic} that is encoded as a graph, and use it for large-scale planning. Different examples in the literature \cite{eysanbach2019sorb, wu2019bayesian, emmons2020sparse, wiyatno2022lifelong, 
meng2020scaling, kwon2021vgm, chaplot2020NTS, shah2021ving, savinov2018sptm, bansal2020combining} use this topological memory as a \textit{global planner} to obtain navigation waypoints towards a goal and a \textit{local policy} to navigate towards these waypoints. However, these methods have two significant limitations. Firstly, spurious connections in the graph can adversely affect the planner's ability to derive a feasible plan (e.g., connections that allow warping between obstacles). Secondly, these methods do not scale well in terms of memory as the number of vertices in the graph scale with the size of the environment.

These limitations are partially addressed by hand-crafted heuristics. Examples of these include connectivity thresholds to prune the number of spurious edges \cite{savinov2018sptm, eysanbach2019sorb}, node sparsification strategies \cite{emmons2020sparse, bansal2020combining} and lifelong updates to the graph \cite{wu2019bayesian, wiyatno2022lifelong}. However, these methods end up adding a non-negligible amount of parameters that require tuning and are often environment-dependant. In contrast, our method avoids the need for such heuristics by utilizing a locomotion head that connects vertices using their latent representation, which we explicitly encourage to be locally consistent. We address the memory issue by embedding the topology of the graph in a geometrically-consistent manner in the weights of the geodesic regressor, similar to \cite{yang2020plan2vec}.

Of particular interest to this work are Semi-Parametric Topological Memory (SPTM) \cite{savinov2018sptm} and Visual Navigation with Goals (ViNG) \cite{shah2021ving}. SPTM utilizes a classifier to determine the connectivity between two temporally close images and creates an unweighted graph based on this. Nevertheless, this graph does not accurately reflect the distance between two infinitely close or distant samples, exacerbating the spurious edges issue. Similarly, ViNG uses a classifier to estimate the temporal number of steps between samples and weight the edges of the graph with these estimates. Both methods employ pruning and sparsification strategies. Our method does not prune the graph and directly estimate the action between two samples, allowing to estimate connectivity and local controls simultaneously. 

Additionally, both SPTM and ViNg create a graph using \textit{all} training images and produce navigation plans by querying the graph using the Dijkstra algorithm \cite{dijkstra1959note}. In contrast, we use our locally consistent latent codes to weight the graph and further embed it in the geodesic regressor, enabling the estimation of shortest path distances over both seen and unseen images in an environment. Drawing inspiration from potential fields planners \cite{choset2005principles}, we employ the geodesic regressor as a potential function and formulate navigation as a minimization problem. This problem can be efficiently solved by utilizing the geodesic regressor in conjunction with forward dynamics, removing the need of expensive graph search queries.

There has also been extensive research on alternative memory representations for embodied navigation, including the use of semantic \cite{georgakis2022learningsemantic, Ramakrishnan2022PONIPF, kim2022topological, wei2019prios} and spatial \cite{gupta2017cognitive, chaplot2020activeslam, henriques2018mapnet} representations. While some methods have already embedded the memory of the problem in neural networks \cite{kuan2019memory}, to the best of our knowledge none of these representations exploit the geometry of the graph to produce a \textit{geometrically consistent} representation. Our approach is inspired by Plan2Vec \cite{yang2020plan2vec} which is a purely planning method. In contrast, our architecture serves for embodied navigation. We learn the geodesic regressor (also known as global metric) on top of our local backbone instead of learning it from scratch. This approach demonstrates that the geometry of the space can be estimated solely from a graph weighted with locally consistent estimates.

Finally, several existing methods rely on having access to relative pose information in order to learn temporal estimates \cite{shah2021ving, bansal2020combining, wiyatno2022lifelong, meng2020scaling}. Our method can be trained in a self-supervised manner using only raw RGB image samples and actions, making it independent of pose information. This capability enables our method to be readily scaled to accommodate large-scale datasets \cite{shah2022lmnav}; however, this aspect will be pursued in future work.

% \textit{experiental learning for navigation} \cite{Levine2023survey}

% general survey learning-based motion planning \cite{wang2021survey}

% Difference between point-nav and image-goal \cite{anderson2018spl}

% Method that has embedding memory instead of topological - it is a semantic method
% \cite{kuan2019memory, kim2022topological}. Recall learning semantic actually have a graph but process it with GNN

% References point-goal \cite{erik2019ddppo, mishkin2019benchmark, chiang2019autorl, emmons2020sparse, bansal2020combining, faust2018prmrl, chaplot2020activeslam}

% Semantic map and object goal \cite{georgakis2022learningsemantic, Ramakrishnan2022PONIPF, kim2022topological, wei2019prios, chang2020youtube}

% image-goal semi-parametric \cite{wiyatno2022lifelong, 
% wu2019bayesian, meng2020scaling, eysanbach20149sorb, kwon2021vgm, chaplot2020NTS, shah2021ving, savinov2018sptm}

% Navigation potential function \cite{choset2005principles}

% Generate graph on the fly but semi-parametric \cite{shah2022viking, shah2021rapid}

% GNM is image-goal
% Latest in the field \cite{shah2022lmnav, shah2022revind, shah2022gnm}

% \cite{yang2020plan2vec} Duh

% Most of these methods share in common a memory representation to achieve the task at hand but none build a geometric memory representation.


% \sm{Discuss learning for navigation. Pointnav vs. imagegoal vs. semantic. Learning is useful vs. classical for RGB and learning non-geometric concepts (TALL GRASS).}
% \sm{Detailed Paragraph on SPTM and ViNG (most closely related methods).}

% Plan2vec \cite{yang2020plan2vec}. Mention isomap. \ms{In manifold learning parlance, the function $\local$ embeds the data manifold $\rgbmanifold$ in a n-dimensional space that locally resembles an n-dimensional euclidean space equipped with a metric $d_{\local}$ [ADD THIS IN RELATED WORK - CONNECTION TO MANIFOLD LEARNING]}.

==> figures/hyperparams_table.tex <==
\begin{table*}
\medskip
\centering
\caption{}
\setlength{\tabcolsep}{6pt}
\begin{tabularx}{\textwidth}{ccccX}
\toprule
 \textbf{Method} & \textbf{Component} & \textbf{Parameter} & \textbf{Value} & \multicolumn{1}{c}{\textbf{Description}} \\
\midrule
\multirow{12}{*}{\textbf{SPTM}} & \multirow{2}{*}{\makecell{Retrieval \\ $R$}} & $l$ & 10 & Maximum temporal distance (steps) between two positive samples. \\
 & & M & 5 & Temporal margin ($l\times$M) between positive and negative samples. \\
\cmidrule(lr){2-5}
 & \multirow{5}{*}{\makecell{Graph \\ $\mathcal{G}$}} & $s_{shortcut}$ & 0.7 & Similarity threshold to create visual shortcut in the graph. \\
 & & \multirow{2}{*}{$\Delta T_l$} & \multirow{2}{*}{5} & Minimum temporal distance between consecutive samples for visual shortcuts. \\
 & & \multirow{2}{*}{$\Delta T_w$} & \multirow{2}{*}{10} & Number of samples in sequence to consider while performing visual shortcuts. \\
\cmidrule(lr){2-5}
 & \multirow{5}{*}{Navigation} & $k$ & 5 & Number of nearest neighbors used to localize new sample in the graph. \\
 & & $s_{local}$ & 0.7 & Threshold used to perform only local localization. \\
 & & $s_{reach}$ & 0.7 & Reachability threshold to pick next navigation waypoint. \\
 & & $H_{min}$ & 1 & Lower interval in the search window for next navigation waypoint.  \\
 & & $H_{max}$ & 20 & Upper interval in the search window for next navigation waypoint. \\
\midrule
\multirow{4}{*}{\textbf{ViNG}} & \multirow{2}{*}{\makecell{Traversability \\ $\mathcal{T}$}} & \multirow{2}{*}{$d_{max}$} & \multirow{2}{*}{20} & Maximum temporal distance (steps) between two samples the model is capable to predict. \\
\cmidrule(lr){2-5}
 & \makecell{Graph \\ $\mathcal{G}$} & $\delta_{sparsify}$ & 5.0 & Sparsification threshold for easily traversable vertices in the graph \\
\midrule
\multirow{8}{*}{\textbf{O4A}} & \multirow{2}{*}{\makecell{Local Backbone \\ $\local$}} & $\posmargin$ & 1 & Positive margin for siamese loss used to train local backbone. \\
 & & $\negmargin$ & 10 & Negative margin for siamese loss used to train local backbone. \\
\cmidrule(lr){2-5}
 & \multirow{6}{*}{Navigation} & \multirow{2}{*}{$m_r$} & \multirow{2}{*}{2.5} & Radius at which the repulsors are activate with respect to current observation. \\
 & & \multirow{2}{*}{$\mathtt{thresh}$} & \multirow{2}{*}{3.5} & Minimum local metric distance between current observation and goal to call $\mathtt{STOP}$. \\
 & & \multirow{2}{*}{$|\mathcal{B}|$} & \multirow{2}{*}{500} & Maximum number of previously visited states stored and used for the repulsor function. \\
\bottomrule
% \vspace{-7.0mm}
\end{tabularx}
\label{table:table_main}
\end{table*}
